The NANOGrav 15-year Data Set: Observations and Timing of 68 Millisecond Pulsars

We present observations and timing analyses of 68 millisecond pulsars (MSPs) comprising the 15-year data set of the North American Nanohertz Observatory for Gravitational Waves (NANOGrav). NANOGrav is a pulsar timing array (PTA) experiment that is sensitive to low-frequency gravitational waves. This is NANOGrav's fifth public data release, including both "narrowband" and "wideband" time-of-arrival (TOA) measurements and corresponding pulsar timing models. We have added 21 MSPs and extended our timing baselines by three years, now spanning nearly 16 years for some of our sources. The data were collected using the Arecibo Observatory, the Green Bank Telescope, and the Very Large Array between frequencies of 327 MHz and 3 GHz, with most sources observed approximately monthly. A number of notable methodological and procedural changes were made compared to our previous data sets. These improve the overall quality of the TOA data set and are part of the transition to new pulsar timing and PTA analysis software packages. For the first time, our data products are accompanied by a full suite of software to reproduce data reduction, analysis, and results. Our timing models include a variety of newly detected astrometric and binary pulsar parameters, including several significant improvements to pulsar mass constraints. We find that the time series of 23 pulsars contain detectable levels of red noise, 10 of which are new measurements. In this data set, we find evidence for a stochastic gravitational-wave background.

==> table_propermotion_changes.tex <==
\begin{deluxetable*}{ccccccc}
\tabletypesize{\scriptsize}
\tablewidth{\textwidth}
\tablecolumns{7}
\tablecaption{Significant Changes in Components of Proper Motion\tablenotemark{\scriptsize{a}} \label{tab:DeltaPM}}
%
\tablehead{\colhead{PSR Name} & \colhead{$\mu_{\lambda, 12.5}$}& \colhead{$\mu_{\lambda, 15}$} & \colhead{$\Delta\mu_{\lambda}/\sigma_{12.5}$} & \colhead{$\mu_{\beta, 12.5}$} & \colhead{$\mu_{\beta, 15}$} & \colhead{$\Delta\mu_{\beta}/\sigma_{12.5}$}
}
\startdata
%
B1937+21 & $-$0.018(4) & $-$0.027(2) & 2.2 & \cdots{} & \cdots{} & \cdots{} \\
%
J0023+0923 & \cdots{} & \cdots{} & \cdots{} & $-$0.70(17) & $-$0.41(9) & 1.8 \\
%
J0340+4130 & $-$1.34(6) & $-$1.47(3) & 2.2 & \cdots{} & \cdots{} & \cdots{} \\
%
J0613$-$0200 & 2.13(1) & 2.1067(60) & 2.5 & \cdots{} & \cdots{} & \cdots{} \\
%
J0636+5128 & 3.325(40) & 3.19(2) & 3.5 & $-$1.4(1) & $-$1.665(45) & 2.1 \\
%
J1713+0747 & 5.268(2) & 5.263(1) & 2.8 & \cdots{} & \cdots{} & \cdots{} \\
%
J1741+1351 & $-$8.66(1) & $-$8.684(6) & 2.0 & $-$7.79(2) & $-$7.822(9) & 1.5 \\
%
J1909$-$3744 & $-$13.862(2) & $-$13.870(1) & 3.7 & \cdots{} & \cdots{} & \cdots{} \\
%
J1911+1347 & $-$3.47(2) & $-$3.438(8) & 1.9 & \cdots{} & \cdots{} & \cdots{} \\
%
J1946+3417 & $-$5.9(1) & $-$5.1(1) & 7.0 & 6.70(16) & 7.01(15) & 2.0 \\
%
J2043+1711 & $-$8.815(9) & $-$8.8287(35) & 1.5 & \cdots{} & \cdots{} & \cdots{} \\
%
J2145$-$0750 & \cdots{} & \cdots{} & \cdots{} & $-$4.7(3) & $-$5.3(2) & 2.1 \\
%
J2229+2643 & \cdots{} & \cdots{} & \cdots{} & $-$4.34(8) & $-$4.50(3) & 2.1 \\
%
J2234+0944 & \cdots{} & \cdots{} & \cdots{} & $-$32.3(2) & $-$32.7(1) & 2.2 \\
\enddata
\tablenotetext{\scriptsize{a}}{The table lists the components of proper motion in ecliptic longitude ($\mu_{\lambda}$) and latitude ($\mu_{\beta}$) from the 12.5-yr and 15-yr data sets, as well as magnitude of the change between the two data sets compared to the uncertainty from \twelveyr ($\sigma_{12.5}$). Only parameters that have changed by $\gtrsim 1.5\sigma_{12.5}$ are listed.}
\end{deluxetable*}
